Supporting Safety Analysis of Image-processing DNNs through Clustering-based Approaches

The adoption of deep neural networks (DNNs) in safety-critical contexts is often prevented by the lack of effective means to explain their results, especially when they are erroneous. In our previous work, we proposed a white-box approach (HUDD) and a black-box approach (SAFE) to automatically characterize DNN failures. They both identify clusters of similar images from a potentially large set of images leading to DNN failures. However, the analysis pipelines for HUDD and SAFE were instantiated in specific ways according to common practices, deferring the analysis of other pipelines to future work. In this paper, we report on an empirical evaluation of 99 different pipelines for root cause analysis of DNN failures. They combine transfer learning, autoencoders, heatmaps of neuron relevance, dimensionality reduction techniques, and different clustering algorithms. Our results show that the best pipeline combines transfer learning, DBSCAN, and UMAP. It leads to clusters almost exclusively capturing images of the same failure scenario, thus facilitating root cause analysis. Further, it generates distinct clusters for each root cause of failure, thus enabling engineers to detect all the unsafe scenarios. Interestingly, these results hold even for failure scenarios that are only observed in a small percentage of the failing images.

==> RQ2_SAFE.tex <==
\subsubsection{RQ2} \emph{How does \APPR compare to DNN accuracy improvement practices supported by HUDD and baseline methods?}
\label{sec:rq2}



\vspace{1mm}
\emph{Design and measurements.} 
In this experiment, we investigate whether \APPR significantly improves the accuracy due to retraining the DNN, thanks to its selection method accounting for the shape of clusters. We compare these improvements to HUDD and two baselines, namely BL1 and BL2, which are depicted in Figure~\ref{fig:baselines} and explained in the following:

\textit{BL1}: In this baseline, we use the error-inducing images in the improvement set as an unsafe set.
Precisely, we label\footnote{For our experiments, labeling comes for free because we either derive images using a simulator or we rely on available datasets. However, labeling comes at a high cost in industrial practice, where new images are collected from the field.} a random subset of the improvement set and execute the DNN to identify error-inducing images.
As for HUDD, this selected unsafe set 
is augmented by applying bootstrap resampling (i.e., replicating samples in the unsafe set) in order to have a sufficiently large number of unsafe images to improve the DNN. 

\textit{BL2}: 
This baseline consists of randomly selecting a set of images from the improvement set, labeling them to obtain a \emph{labeled selected improvement set}, and using them for retraining.

 \begin{figure}[htp]
\includegraphics[width=\textwidth]{images/baselines.pdf}
\caption{Process of the two baselines used to compare \APPR}
\label{fig:baselines}
\end{figure}

We rely on the same settings and environment to run the experiments for the four different retraining strategies (i.e., SAFE, HUDD, BL1, and BL2). These experiments are repeated ten times to account for randomness.

 

To retrain DNNs, we rely on the approach described in section \ref{sec:step4}. 
\ASEnn{For fair comparisons with HUDD~\cite{fahmysupporting}, BL1, and BL2, we configure bootstrap resampling to generate an \emph{augmented labeled unsafe set} and an \emph{augmented labeled selected improvement set} with the same size as the \emph{balanced labeled unsafe set} for HUDD (see Figure~\ref{fig:HUDD}).}

We compute the accuracy of the retrained models on the test sets and compare the accuracy improvement obtained by \APPR with those obtained by HUDD and the baselines. For this experiment, we consider the case study subjects presented in Table \ref{tab:dnns}.

The improvement sets for \GD and \CloseDNN have been generated through additional executions of UnityEyes.
For \HPD and \FLD, they have been generated with additional executions of the IEE simulator, configured to use two new face models which were not used for generating the training and test sets.
We selected images of the original datasets not used for the training and test sets for the other cases.




 



\emph{Results.} Table~\ref{tab:rq2_safe} provides an accuracy comparison between \APPR, HUDD, and the two baselines on the different case study DNNs. It also provides the size of the unsafe sets (number of images) selected by each method. 

\input{tables/RQ2_results}
\input{tables/VDA_results2}

For \APPR, improvements in accuracy over the original model varies from 0.79 to 34.18, compared to lower ranges for HUDD (from 0.28\% to 30.24\%), BL1 (from -0.18\% to 27.03\%) and BL2 (-0.15\% to 28.84\%). Across case study DNNs, \APPR clearly and systematically yields better accuracy results compared to HUDD and the baselines, though to varying extents. Note that unsafe set sizes are comparable across improvement strategies and that differences in accuracy are therefore due to the strategy adopted for selecting unsafe images.  

The lower improvement shown by the baselines can be explained by the fact they do not rely on root cause clusters to select images for the unsafe set, a strategy that appears to be beneficial in our context.

\APPR always yields higher improvement than that of HUDD. This is because HUDD relies on the cluster's centroids to select images for the unsafe set without accounting for the cluster's shape. In contrast, \APPR relies on core points to choose the images for the unsafe set. This enables the handling of clusters with arbitrary shapes as the selected images take the shape of the cluster, as explained in Section \ref{sec:step4}. %

Regarding \APPR results, we notice three types of improvement explained in the following:

For \GD, the improvement is only +0.79. This is because the accuracy of the original model for this case study subject was already very high (95.95\%), with limited room for improvement.

For \HPD and \FLD, the improvement in accuracy is +26.16 and +34.18, respectively. The original models for these two case study subjects had low accuracy and we therefore expected a large improvement. In fact, \HPD and \FLD represent two cases where retraining was very much needed.

For \CloseDNN, TS and \ODDNN, the improvement in accuracy is +8.2, +11.82 and +13.18, respectively. Though this improvement is moderate compared to the previous case study DNNs, it is still significant given the original models' relatively high accuracy. After retraining, \APPR achieved high accuracy for these case study subjects with 96.29\%, 93.47\%, and 97.30\%, respectively.

We report the significance of these results in Table \ref{vda_results}, including the values of the Vargha and Delaney's $\hat{A}_{12}$ effect size and the p-values resulting from performing a Mann-Whitney U-test between the accuracy of \APPR and other improvement strategies. Recall that we run each strategy 10 times. 


Typically, an $\hat{A}_{12}$ effect size above 0.56 is considered significant with higher thresholds for medium (0.64) and large (0.71) effects, thus suggesting the effect sizes between \APPR and other strategies are large across case study DNNs, in all but one case. 

We notice in Table \ref{vda_results} that the p-values when comparing \APPR to the baselines are always below 0.05. As for HUDD, the p-values are lower than 0.05 in 5 out of 6 case study subjects. This implies that in most cases, the null hypothesis is rejected. 


\input{tables/execution_time}


In conclusion, \APPR proved its effectiveness in retraining the different case study subjects as it obtained significant improvements over the original models. \APPR not only performs better than HUDD but also, and perhaps more significantly, provides very high time and memory savings. We report in Table~\ref{tab:execution_time} the time required to extract the features by \APPR and to generate the heatmaps by HUDD; we do not report the time required to perform the other steps of the two approaches because these steps are either shared or do not have any practical impact on performance (i.e., they took few seconds in our experiments). We also report the memory allocation of the features and the heatmaps, which are the data types processed only by \APPR and HUDD, respectively. We observe a large time and memory saving for \APPR compared to HUDD. Such performance considerations have significant practical implications. For example, we can observe that SAFE requires, in the worst case, only 3.5 minutes to generate RCCs and the unsafe set to be used for retraining. HUDD, instead, requires 65 minutes to achieve the same objective. Such difference has a huge impact on the practicality of the approach as, for SAFE, the analysis of RCCs can be performed shortly after observing DNN failures. HUDD may require up to one hour to do the same. %
Such execution time savings allow engineers to conduct DNN safety analysis and improvements in a much shorter time. Memory savings also have significant implications since it prevents the need for expensive hardware to perform such analysis.  

The explanation for the above results is that \APPR is using extracted features to represent the images instead of heatmaps. Feature extraction is less costly in time and memory than the computation of heatmaps. Indeed, the distance computed on features is less computationally complex than the one calculated on heatmaps. 

Heatmaps also take a great deal of memory for storage. HUDD generates heatmaps for each layer. For instance, the heatmap for the eighth layer of AlexNet has a size of $169 \times 256$ (convolution layer), while the heatmap for the tenth layer has a size of $4096 \times C$. With this architecture, HUDD will generate eight heatmaps of size $169 \times 256$ and one heatmap of size $4096 \times C$ for every image in the dataset. In contrast, for \APPR, each image is represented by a $1 \times 256$ matrix (256 features for each image).


==> notes.tex <==

\subsection{Background notes by Mohammed}
\subsection{Computer Vision}
	Computer vision is a field of artificial intelligence. It allows computers to analyze, process, and understand images. Computer vision systems are employed to extract relevant data from visual inputs to use them in other recommendation tasks.
	
	In recent years, convolutional neural networks (CNNs) have attracted much attention from the computer vision community. This success is related to different factors, such as the impressive error rate achieved by the AlexNet architecture \cite{krizhevsky2012imagenet}, the massive amounts of accessible data, and the availability of powerful graphics processing units (GPU).
	CNNs are characterized by their capacity to learn data representation compared to traditional machine learning methods. In these architectures, the feature extraction process is performed based on convolutional layers instead of using handcrafted features.
	
	To optimize the traditional CNN architecture, various structures have been proposed \cite{simonyan2014very,szegedy2015going,szegedy2016rethinking,he2016deep,howard2017mobilenets}. The main purpose was to develop deeper architectures while reducing the number of trainable parameters. VGGNet \cite{simonyan2014very} proposes the exploitation of convolutional layers associated with small receptive fields ($3 \times 3$). Inception \cite{szegedy2015going} use Inception modules instead of the standard convolutional layers \footnote{The main difference between the VGGNet and the InceptionV3 architectures is the nature of convolutional layers. VGGNet is based on the standard convolutional layers. In contrast, InceptionV3 exploit Inception blocks, where each Inception module regroups many convolutions.}. Combining these modules has successfully generated a deep network (22 layers) that reduces 12 times the number of the AlexNet's parameters \cite{krizhevsky2012imagenet}. ResNet \cite{he2016deep} introduces residual connections between convolutional layers to avoid the gradient vanishing problem. Finally, other architectures such as MobileNetV1 \cite{howard2017mobilenets} and  MobileNetV2  \cite{sandler2018mobilenetv2} have been developed for mobile and embedded vision applications.
	
	Despite their ability to learn data representation, DL networks require huge volumes of data to prevent overfitting problems. Datasets characterized by reduced volumes of data, limit the efficiency of CNNs in the classification process. As a solution, the transfer learning technique has been largely considered. This method transfers the knowledge from a generic domain, usually ImageNet, to another specific domain.
	
	\subsection{Feature extraction}
	The purpose of feature extraction is to transform unstructured data into structured raw data for their exploitation by clustering algorithms. In this study, we extracted features based on convolutional neural networks (CNNs). The standard  CNN architecture is composed of three types of layers: convolutional layers, pooling layers, and fully connected (FC) layers. 
	
	The convolutional layer is considered as the primary building block of a CNN. This layer extracts relevant features from input images during training. Besides, pooling layers are used for dimensionality reduction. Convolutional and pooling layers are stacked to form a hierarchical feature extraction module. The resulted feature map from the last pooling layer is presented as a 3D matrices of size (N, N, Nc), where N is the width and the height of the pooling layer, and Nc is its depth. For features extraction, this feature map is flattened to form a vector of size (1, $N \times N $). To resume, the CNN model receives an input image of size $(224,224,3)$. This image is then forwarded through the network's layers to generate a vector of features. The feature extraction process from all images generates a raw data represented by a 2D matrix (denoted as X), $l_i$ represent the  class categories, X and $l_i$ can be described as:  
	{
		\begin{equation}
			X = \begin{bmatrix}
				x_{11} & x_{12}  & ...  &   x_{1m} & l_2\\ 
				x_{21} &  x_{22}  & ...  & x_{2m} & l_c \\ 
				... & ...   & ...   & ...  & ... \\ 
				x_{k1} & x_{k2}  & ...  & x_{km} & l_1 \\
			\end{bmatrix}, l_i \in \left \{ l_1,l_2,...,l_{c}  \right \}, i \in [1,c] 
		\end{equation}
	}
	Where, c is the number of categories, $m = N \times N $ is the number of features, and k is the number of samples in the dataset. 
	
	In this study, we used VGG16 as a feature extraction CNN architecture. However, several CNNs architectures for feature extraction exists: InceptionV3 \cite{szegedy2015going}, VGG19 \cite{simonyan2014very}, ResNet50 \cite{ he2016deep}, and MobileNet \cite{howard2017mobilenets}. We exploited the pre-trained models on the ImageNet dataset, since, unlike the traditional feature extraction methods, CNNs must be pre-trained to perform feature extraction.  The number of extracted features is related to the used architecture, where InceptionV3, VGG16, VGG19, ResNet50, and MobileNet generated 2048, 512, 512, 2048, and 1024 features, respectively. 
	In the following sections we describe the most used CNN architectures for features extraction.
	\subsection{VGGNet}
	VGGNet \cite{simonyan2014very} is a convolutional neural network characterized by deep configurations (16 to 19 layers). The purpose of this architecture is to increase the network's depth and to minimize the number of trainable parameters.  Controlling the number of parameters helps to reduce overfitting issues. To this end,  VGGNet proposes to decrease the size of filters from $7 \times 7$ and $5 \times 5$ to $3 \times 3$. The comparative study between the number of parameters in 3 stacked convolutional layers associated with $3 \times 3$ filters and a single convolutional layer associated with $7 \times 7$   filters demonstrated that small filters reduce the total number of parameters. The number of parameters in 3 stacked convolutional layers ( $3 \times 3$ filters)  is  $3^2C^2$, on the other hand, the number of parameters in a single convolutional layer ( $7 \times 7$ filters) is $7^2C^2$, where, C is the depth of the convolutional layers. 

	To resume, VGGNet proposes to stack convolutional layers associated with small receptive fields to reduce the number of parameters and enhance non-linearity through ReLu activation functions in intermediate layers.    

	VGGNet proposes six different configurations: A, A-LRN, B, C, D, and E, where the depth varies from 11 to 19 layers. In this contribution, we exploited the configurations D and E, which are composed of 16 and 19 layers, respectively. 
	
	\subsection{InceptionV3}
	
	InceptionV3 \cite{szegedy2015going} is a refined version of Inception \cite{szegedy2016rethinking}. This network proposes other variants of Inception blocks to reduce the number of multiplications in the convolution and optimize computational complexity. These variants are based on two types of factorizations: factorization into smaller convolutions and factorization into asymmetric convolutions.  

	The standard Inception blocks use filters with a variable size ($1 \times 1$, $3 \times 3$, and $5 \times 5$)  in the same convolution instead of using a single filter's size ($3 \times 3$). The results of each filter are then stacked and considered as an input to the next convolutional layer. Using multiple filters in the same convolution helps to avoid patch alignment problems.

	The factorization into smaller convolutions proposes reducing the filter size in the standard convolutions from $5 \times 5$ to $3 \times 3$. This technique replaces $5 \times 5$ filters by two $3 \times 3$  filters to reduce the number of parameters in an Inception block by 25\%.
	
	The factorization into asymmetric convolutions propose to replace $F \times F$ convolutions by asymmetric convolutions associated with $F \times1$ and $1 \times F$ filters. This technique reduces the computational complexity by 33\% for F=3. 

	In addition to the factorization strategy, InceptionV3 exploit other techniques such as label smoothing and auxiliary classifiers.

	To resume, the InceptionV3 architecture is composed of three types of Inception blocks: A, B, C, and C that exploit different factorization techniques.
	\subsection{ResNet}
	ResNet \cite{ he2016deep} is a convolutional neural network based on residual blocks. The purpose of this architecture is to solve vanishing gradient problems in deep neural networks. During the backpropagation process, the gradient diminishes dramatically in deep networks. Small values of gradients prevent the weights from changing their values, which slow the training process. To solve this issue, ResNet introduces residual blocks. These buildings blocks present skip connections between the previous convolutional layer's input and the current convolutional layer's output. 

	ResNet proposes different configurations inspired by the VGGNet network. The depth of these configurations varies between 18 and 152 layers. We exploited the ResNet configuration with 50 layers (ResNet50) as a feature extractor in this contribution. 
	\subsection{MobileNet}
	MobileNet \cite{howard2017mobilenets} is a convolutional neural network that has been designed for mobile and embedded vision applications. This architecture is based on depthwise separable convolutions (DSC). The purpose of these buildings blocks is to reduce the number of parameters and optimize computational complexity. DSC factorize a convolution into a depthwise convolution (DC) and a pointwise convolution (PC). Unlike the standard convolutions, in DSC, a single filter is applied to each input channel. Then, the resulted channels are combined by a pointwise convolution. This process reduces the number of parameters by $\frac{1}{N} + \frac{1}{{D_k}^2}$, where $ D_k$ is the size of the filter and N is the number of filters. To construct smaller and computationally less expensive models, MobileNet introduces two hyperparameters: resolution and width multipliers. The purpose of width multiplier ($\alpha \in  \left[ 0, 1\right]$)  is to reduce the number of channels in a convolutional layer from M to $\alpha M$. Besides, the resolution multiplier reduces the computational complexity by decreasing the resolution of the input image. MobileNet is composed of 28 layers: 14 standard convolutional layers, 13 DSC, and one hidden FC. 

\subsection{Fine Tuning}
The pre-trained model on the ImageNet dataset was then used as a base model for transfer learning. Transfer learning reuses a trained model on a source task $ T_S $ on another target task $ T_T $. This technique is performed in two main steps: the network's initialization and fine-tuning. First, we initialized the new VGG16 model by the pre-trained weights P($X_s \mid Y_s$) on the ImageNet dataset instead of random initializations. We subsequently replaced the last softmax layer with a new FC layer composed of C neurons, where C is the number of labels in the target task. Finally, a subset of the first layers is frozen ($l_i \in \left\{1,...,K\right\}; K < L$), whereas, the remaining layers ($l_i \in \left\{K+1,...,L\right\}$ ; L is the number of layers) are fine-tuned on the new target task to obtain the new weights P($X_T \mid Y_T$).
\subsection{Dimensionality Reduction}
Given an instance $X_i$ which is composed of a $a$ vector of a attributes $X_i$ = $x_i^1$ , . . . , $x_i^a$ . The Dimensionality Reduction comprises the process of finding some transformation function (or map) $A$ : $\mathbb{R}^a  \rightarrow \mathbb{R}^m$, where $m < a$, to be applied on each instance $X_i$ as follows:
$Y_i$ = $A(X_i)$,
where $Y_i$ = $y_i$,...,$y_i$.


We distinguish two main different dimensionality reduction categories: (i) feature selection which consists in selecting a subset of the input features, i.e., the most relevant and non-redundant features, without operating any sort of data transformation; and (ii) feature transformation – also called feature extraction – which consists in constructing from a set of input features in high-dimensional space, a new set of features in a lower dimensional space. We used this category for our method.
\subsection{Clustering}
	Clustering is an unsupervised learning technique that divides a set of objects into clusters such that : (a) objects in the same cluster must be similar as much as possible, (b) objects in different clusters must be different as much as possible. In this work, we used DBSCAN clustering algorithm after extensive experiments on several clustering algorithms.
\subsubsection*{DBSCAN clustering Algorithm}	
DBSCAN (density-based spatial clustering of applications with noise) \cite{ester1996density} is the most used density-based clustering algorithm. It considers the points with the most neighbors as centers of the clusters (the regions with high density are considered clusters). At the same time, points with fewer neighbors are considered noise. The DBSCAN algorithm introduces two concepts of Clustering: Reachability and Connectivity.
\begin{itemize}
    \item Reachability: a point is reachable from another if the distance between them is inferior to a threshold $\epsilon$.
    \item Connectivity: if two points $p$ and $q$ are connected they belong to the same cluster. If points $p$ and $r$ are connected and $r$ and $q$ are connected, then $p$ and $q$ are also connected (transitivity). 
\end{itemize}
To apply these concepts, DBSCAN introduces two parameters: $MinPts$ and $\epsilon$.

\begin{itemize}
    \item $MinPts$: the minimum of points that a region should have to be considered dense.
    \item Threshold $ \epsilon $: a threshold to determine if a point belongs to another point's neighborhood.
\end{itemize} 
Based on the concepts described above, DBSCAN presents three types of points:
\begin{itemize}
    \item Core point:  it has at least $MinPts$ points within a distance of $\epsilon$.
    \item Border point: it is not a core point, but it belongs to at least one cluster. That means that it lies within a distance $\epsilon$ from a core point.
    \item Noise point: it's a point that is not a core point nor a border point.
\end{itemize}
Figure \eqref{dbscan} illustrates DBSCAN's point types.\\
\begin{figure}[h]
			\centerline{\includegraphics[width=0.5\textwidth]{figures/dbscan.png}}
			\caption{\label{dbscan} DBSCAN point types}
\end{figure}  
The DBSCAN algorithm proceed by taking point randomly from the dataset until all points are picked. Then for each point it determines if it's a Core, Border or Noise point based on the parameters $\epsilon$ and $MinPts$. The core point are considered centers of each cluster. The clusters are then expanded by recursively repeating the neighborhood calculation for each neighboring point.  Algorithm \eqref{dbscan_algorithm} present the DBSCAN algorithm. The main problems of DBSCAN are its sensitivity to varying density. It is also not suitable with high dimensional data.

	
\subsection{Proposed Method}	
\subsection{Black Box Approach}
For the Black Box approach, we use a pre-trained neural network to extract a feature vector from images and cluster the images based on how similar the feature vectors are.

The pre-trained model we use is the VGG16 convolutional neural network (CNN), which is considered state-of-the-art for image recognition tasks. We use this model as a feature extractor only, meaning that we remove the final (prediction) layer to obtain a feature vector. The VGG16 architecture is illustrated in Figure \ref{vgg16}.

The first step of our approach is to preprocess the images. We downsample the images from 640x480 to 224x224 so that the dimension is compatible with that required by the pre-trained Imagenet we use for fine-tuning.

After preprocessing the images, we load the VGG16 model and remove the output layer manually. This means that the new final layer is a fully connected layer with $4096$ output neurons. This vector of $4096$ numbers is the feature vector that we use to cluster the images. After removing the final layer, we pass our preprocessed images to the network to get our feature vector through the predict function.

Since our vectors have over 4000 dimensions, it will be costly in time and memory to apply the clustering algorithm directly on that vector. We use a dimensionality reduction method (PCA) to reduce features from 4096 to 100 features.

The final step of our method is to apply the DBSCAN clustering algorithm described above on the final feature vectors. The output is a set of clusters and one cluster containing noise (outliers). 


\begin{figure}[h]
			\centerline{\includegraphics[width=0.5\textwidth]{figures/vgg16.png}}
			\caption{\label{vgg16} VGG16 architecture}
\end{figure}  

\subsection{VGG with Fine Tuning approach}
The white box approach is similar to the black box approach except that here we fine tune the top layers of the VGG16 model to fit our data. we perform the fine tuning process as follows:
\begin{itemize}
    \item Remove the fully connected nodes at the end of the network (i.e., where the actual class label predictions are made).
    \item Replace the fully connected nodes with freshly initialized ones. The number of neurons should correspond to the number of classes in our case study.
    \item Freeze earlier CONV layers earlier in the network (ensuring that any previous robust features learned by the VGG16 are not destroyed).
    \item Start training, but only train the FC layer heads.
\end{itemize}
The idea of the fine tuning is to use a black box method but train the top layers to learn from our case study.

The rest of the approach is similar to the black box method. The process of the proposed method is illustrated in Figure \ref{FE_process}.	
\begin{figure*}[h]
			\centerline{\includegraphics[width=\textwidth]{figures/FE_process.png}}
			\caption{\label{FE_process} Process of the proposed method}
\end{figure*}  	
\subsection{Experimental Results}

\begin{table}[H]
\small
\makebox[\textwidth]{

\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Cluster} & \textbf{Explanatory Parameters}                                                                    & \textbf{Variance Reduction}                                              & \textbf{Average Values}                                                         & \textbf{Unsafe Value}                                                & \textbf{Condition}                                                                                                                                                                                 \\ \hline
1                & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}99\%\\ 98\%\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}202.51\\ 161.79\end{tabular}                         & \begin{tabular}[c]{@{}c@{}}202.5\\ 160\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}191.25 \textless{}\textgreater 213.75\\ 145 \textless{}\textgreater 175\end{tabular}                                                                                    \\ \hline
2                & Angle                                                                                              & 99\%                                                                     & 115.41                                                                          & 112.5                                                                & 101.25 \textless{}\textgreater 123.75                                                                                                                                                              \\ \hline
3                & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\\ V\_Headpose\\ StrangeDist\end{tabular}            & \begin{tabular}[c]{@{}c@{}}99\%\\ 98\%\\ 93\%\\ 88\%\end{tabular}        & \begin{tabular}[c]{@{}c@{}}24.36\\ 205.8\\ 17.96\\ -25\end{tabular}             & \begin{tabular}[c]{@{}c@{}}22.5\\ 220\\ 20\\ -14\end{tabular}        & \begin{tabular}[c]{@{}c@{}}11.25 \textless{}\textgreater 33.75\\ 205 \textless{}\textgreater 235\\ 10 \textless{}\textgreater 30\\ \textless -11.5\end{tabular}                                    \\ \hline
4                & Angle                                                                                              & 99\%                                                                     & 336.1                                                                           & 337.5                                                                & 191.25 \textless{}\textgreater 213.75                                                                                                                                                              \\ \hline
5                & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\\ V\_Headpose\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}99\%\\ 99\%\\ 93\%\end{tabular}               & \begin{tabular}[c]{@{}c@{}}156.66\\ 171.85\\ 15.96\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}157.5\\ 160\\ 20\end{tabular}             & \begin{tabular}[c]{@{}c@{}}146.25 \textless{}\textgreater 168.75\\ 145 \textless{}\textgreater 175\\ 10 \textless{}\textgreater 30\end{tabular}                                                    \\ \hline
6                & \begin{tabular}[c]{@{}c@{}}Angle\\ V\_Headpose\\ StrangeDist\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}99\%\\ 99\%\\ 70\%\end{tabular}               & \begin{tabular}[c]{@{}c@{}}155.94\\ 15.53\\ -22.5\end{tabular}                  & \begin{tabular}[c]{@{}c@{}}157.5\\ 20\\ -14\end{tabular}             & \begin{tabular}[c]{@{}c@{}}146.25 \textless{}\textgreater 168.75\\ 10 \textless{}\textgreater 30\\ \textless -11.5\end{tabular}                                                                    \\ \hline
7                & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\\ V\_Headpose\\ StrangeDist\\ Distance\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 99\%\\ 97\%\\ 71\%\\ 96\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}204.57\\ 170.52\\ 343.19\\ -22.4\\ 21.8\end{tabular} & \begin{tabular}[c]{@{}c@{}}202.5\\ 160\\ 340\\ -14\\ 25\end{tabular} & \begin{tabular}[c]{@{}c@{}}191.25 \textless{}\textgreater 213.75\\ 145 \textless{}\textgreater 175\\ 330 \textless{}\textgreater 350\\ \textless -11.5\\ 4 \textless{}\textgreater 36\end{tabular} \\ \hline
8                & \begin{tabular}[c]{@{}c@{}}Angle\\ StrangeDist\\ Distance\end{tabular}                             & \begin{tabular}[c]{@{}c@{}}99\%\\ 75\%\\ 95\%\end{tabular}               & \begin{tabular}[c]{@{}c@{}}246.19\\ -22.62\\ 21.87\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}247.5\\ -14\\ 25\end{tabular}             & \begin{tabular}[c]{@{}c@{}}236.25 \textless{}\textgreater 258.75\\ \textless -11.5\\ 4 \textless{}\textgreater 36\end{tabular}                                                                     \\ \hline
9                & \begin{tabular}[c]{@{}c@{}}Angle\\ V\_Headpose\end{tabular}                                        & \begin{tabular}[c]{@{}c@{}}99\%\\ 94\%\end{tabular}                      & \begin{tabular}[c]{@{}c@{}}66.98\\ 342.13\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}67.5\\ 340\end{tabular}                   & \begin{tabular}[c]{@{}c@{}}56.25 \textless{}\textgreater 78.75\\ 330 \textless{}\textgreater 350\end{tabular}                                                                                      \\ \hline
10               & \begin{tabular}[c]{@{}c@{}}Angle\\ V\_Headpose\\ StrangeDist\\ Distance\end{tabular}               & \begin{tabular}[c]{@{}c@{}}99\%\\ 92\%\\ 97\%\\ 97\%\end{tabular}        & \begin{tabular}[c]{@{}c@{}}246.15\\ 18.37\\ -22.8\\ 15\end{tabular}             & \begin{tabular}[c]{@{}c@{}}247.5\\ 20\\ -14\\ 25\end{tabular}        & \begin{tabular}[c]{@{}c@{}}236.25 \textless{}\textgreater 258.75\\ 10 \textless{}\textgreater 30\\ \textless -11.5\\ 4 \textless{}\textgreater 36\end{tabular}                                     \\ \hline
11               & Angle                                                                                              & 99\%                                                                     & 113.11                                                                          & 112.5                                                                & 101.25 \textless{}\textgreater 123.75                                                                                                                                                              \\ \hline
12               & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\\ V\_Headpose\end{tabular}                          & \begin{tabular}[c]{@{}c@{}}99\%\\ 90\%\\ 99\%\end{tabular}               & \begin{tabular}[c]{@{}c@{}}247.87\\ 162.08\\ 14.67\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}247.5\\ 160\\ 20\end{tabular}             & \begin{tabular}[c]{@{}c@{}}236.25 \textless{}\textgreater 258.75\\ 145 \textless{}\textgreater 175\\ 10 \textless{}\textgreater 30\end{tabular}                                                    \\ \hline
13               & Angle                                                                                              & 99\%                                                                     & 204.48                                                                          & 202.5                                                                & 191.25 \textless{}\textgreater 213.75                                                                                                                                                              \\ \hline
\end{tabular}
}
\caption{Clusters with at least one explanatory parameter (i.e. close to an unsafe value) for GD dataset}\label{gd_rq13}
\end{table}


\begin{table}[H]
\small
\makebox[\textwidth]{

\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Cluster} & \textbf{Explanatory Parameters}                                             & \textbf{Variance Reduction}                                & \textbf{Average Values}                                         & \textbf{Unsafe Value}                                    & \textbf{Condition}                                                                                                           \\ \hline
1                & \begin{tabular}[c]{@{}c@{}}Distance\\ StangeDist\\ H\_Headpose\end{tabular} & \begin{tabular}[c]{@{}c@{}}84\%\\ 82\%\\ 95\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}28.27\\ -20.36\\ 173.06\end{tabular} & \begin{tabular}[c]{@{}c@{}}25\\ -14\\ 160\end{tabular}   & \begin{tabular}[c]{@{}c@{}}4 \textless{}\textgreater 36\\ \textless -16\\ 145 \textless{}\textgreater 175\end{tabular}       \\ \hline
2                & \begin{tabular}[c]{@{}c@{}}Distance\\ StangeDist\\ V\_Headpose\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 89\%\\ 93\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}21.66\\ -16.33\\ 341.21\end{tabular} & \begin{tabular}[c]{@{}c@{}}25\\ -14\\ 340\end{tabular}   & \begin{tabular}[c]{@{}c@{}}4 \textless{}\textgreater 36\\ \textless -16\\ 330 \textless{}\textgreater 350\end{tabular}       \\ \hline
3                & \begin{tabular}[c]{@{}c@{}}Distance\\ StangeDist\\ V\_Headpose\end{tabular} & \begin{tabular}[c]{@{}c@{}}86\%\\ 82\%\\ 99\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}26\\ -24.66\\ 343.19\end{tabular}    & \begin{tabular}[c]{@{}c@{}}25\\ -14\\ 340\end{tabular}   & \begin{tabular}[c]{@{}c@{}}4 \textless{}\textgreater 36\\ \textless -16\\ 330 \textless{}\textgreater 350\end{tabular}       \\ \hline
4                & \begin{tabular}[c]{@{}c@{}}Distance\\ StangeDist\\ H\_Headpose\end{tabular} & \begin{tabular}[c]{@{}c@{}}98\%\\ 84\%\\ 99\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}34.75\\ -16.75\\ 207.84\end{tabular} & \begin{tabular}[c]{@{}c@{}}25\\ -14\\ 220\end{tabular}   & \begin{tabular}[c]{@{}c@{}}4 \textless{}\textgreater 36\\ \textless -16\\ 205\textless{}\textgreater{}235\end{tabular}       \\ \hline
5                & \begin{tabular}[c]{@{}c@{}}Angle\\ H\_Headpose\end{tabular}                 & \begin{tabular}[c]{@{}c@{}}63\%\\ 96\%\end{tabular}        & \begin{tabular}[c]{@{}c@{}}245.36\\ 171.65\end{tabular}         & \begin{tabular}[c]{@{}c@{}}247.5\\ 160\end{tabular}      & \begin{tabular}[c]{@{}c@{}}236.25\textless{}\textgreater{}258.75\\ 145 \textless{}\textgreater 175\end{tabular}              \\ \hline
6                & \begin{tabular}[c]{@{}c@{}}Distance\\ StangeDist\\ Angle\end{tabular}       & \begin{tabular}[c]{@{}c@{}}98\%\\ 96\%\\ 95\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}29.5\\ -19.25\\ 208.48\end{tabular}  & \begin{tabular}[c]{@{}c@{}}25\\ -14\\ 202.5\end{tabular} & \begin{tabular}[c]{@{}c@{}}4 \textless{}\textgreater 36\\ \textless -16\\ 191.25\textless{}\textgreater{}213.75\end{tabular} \\ \hline
7                & Distance                                                                    & 99\%                                                       & 35.33                                                           & 25                                                       & 4 \textless{}\textgreater 36                                                                                                 \\ \hline
\end{tabular}
}
\caption{Clusters with at least one explanatory parameter (i.e. close to an unsafe value) for OC dataset}\label{oc_rq13}
\end{table}


\begin{table}[H]
\small
\makebox[\textwidth]{
\begin{tabular}{|c|c|c|c|c|c|}
\hline
\textbf{Cluster} & \textbf{Explanatory Parameters}                                   & \textbf{Variance Reduction}                         & \textbf{Average Values}                                 & \textbf{Unsafe Value}                             & \textbf{Condition}                                                                                              \\ \hline
1                & Headpose\_X                                                       & 57\%                                                & -28,29                                                  & -28.88                                            & -28.88\textless{}\textgreater{}-24.16                                                                           \\ \hline
2                & Headpose\_X                                                       & 99\%                                                & 67                                                      & 74                                                & 42\textless{}\textgreater{}74                                                                                   \\ \hline
3                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}93\%\\ 95\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}11.98\\ -0.63\end{tabular}   & \begin{tabular}[c]{@{}c@{}}10\\ 0\end{tabular}    & \begin{tabular}[c]{@{}c@{}}7.5\textless{}\textgreater{}12.5\\ -2.5\textless{}\textgreater{}2.5\end{tabular}     \\ \hline
4                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 98\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}-0.47\\ -0.48\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0\\ 0\end{tabular}     & \begin{tabular}[c]{@{}c@{}}-2.5\textless{}\textgreater{}2.5\\ -2.5\textless{}\textgreater{}2.5\end{tabular}     \\ \hline
5                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}95\%\\ 90\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}-1.8\\ -21.7\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0\\ -10\end{tabular}   & \begin{tabular}[c]{@{}c@{}}-2.5\textless{}\textgreater{}2.5\\ -29.5\textless{}\textgreater{}-5.5\end{tabular}   \\ \hline
6                & Headpose\_Y                                                       & 99\%                                                & -1.63                                                   & 0                                                 & -2.5\textless{}\textgreater{}2.5                                                                                \\ \hline
7                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 92\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}0.53\\ -22.7\end{tabular}    & \begin{tabular}[c]{@{}c@{}}0\\ -10\end{tabular}   & \begin{tabular}[c]{@{}c@{}}-2.5\textless{}\textgreater{}2.5\\ -29.5\textless{}\textgreater{}-5.5\end{tabular}   \\ \hline
8                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 99\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}-0.19\\ -2.28\end{tabular}   & \begin{tabular}[c]{@{}c@{}}0\\ 0\end{tabular}     & \begin{tabular}[c]{@{}c@{}}-2.5\textless{}\textgreater{}2.5\\ -2.5\textless{}\textgreater{}2.5\end{tabular}     \\ \hline
9                & \begin{tabular}[c]{@{}c@{}}Headpose\_X\\ Headpose\_Y\end{tabular} & \begin{tabular}[c]{@{}c@{}}99\%\\ 99\%\end{tabular} & \begin{tabular}[c]{@{}c@{}}-11.01\\ -16.61\end{tabular} & \begin{tabular}[c]{@{}c@{}}-10\\ -10\end{tabular} & \begin{tabular}[c]{@{}c@{}}-14.5\textless{}\textgreater{}-5.5\\ -29.5\textless{}\textgreater{}-5.5\end{tabular} \\ \hline
10               & Headpose\_Y                                                       & 98\%                                                & -1.67                                                   & 0                                                 & -2.5\textless{}\textgreater{}2.5                                                                                \\ \hline
\end{tabular}
}
\caption{Clusters with at least one explanatory parameter (i.e. close to an unsafe value) for HPD dataset}\label{hpd_rq13}
\end{table}


Comparison between HUDD and FE in:
\begin{itemize}
\item Percentage of clusters with at least one parameter with reduction in variance above 50\%
\item Percentage of clusters with at least one explanatory parameter

\end{itemize}

\begin{table}[H]
\small
\makebox[\textwidth]{
\begin{tabular}{|c|c|c|c|c|}
\hline
\textbf{Case Study} & \multicolumn{2}{c|}{\textbf{HUDD}}      & \multicolumn{2}{c|}{\textbf{Feature Extraction}} \\ \hline
                    & Reduced Clusters & Explanatory Clusters & Reduced Clusters      & Explanatory Clusters     \\ \hline
GD                  & 100\%            & 86\%                 & 100\%                 & 100\%                    \\ \hline
OC                  & 57\%             & 57\%                 & 100\%                 & 100\%                    \\ \hline
HPD                 & 100\%            & 88\%                 & 100\%                 & 100\%                    \\ \hline
\end{tabular}
}
\caption{Comparison between HUDD and FE methods) for HPD dataset}\label{hudd_vs_fe}
\end{table}



==> tables/execution_time.tex <==
\begin{table}[t]
\caption{Execution time of the feature extraction of the improvement sets and the memory allocations of these features for \APPR. Compared to the execution time of the generation of the heatmaps and their memory allocation.}
\label{tab:execution_time}
\footnotesize
\makebox[0.5\textwidth]{\begin{tabular}{|c|cc|cc|}
\hline
Subject& \multicolumn{2}{c|}{Execution time (s)} & \multicolumn{2}{c|}{Memory allocation (Mb)} \\ \hline
           & \multicolumn{1}{c|}{SAFE}     & HUDD    & \multicolumn{1}{c|}{SAFE}       & HUDD      \\ \hline
GD         & \multicolumn{1}{c|}{176}      & 3,920   & \multicolumn{1}{c|}{74.2}       & 78,641  \\ \hline
OC         & \multicolumn{1}{c|}{160}      & 958     & \multicolumn{1}{c|}{4.1}        & 3,551    \\ \hline
HPD        & \multicolumn{1}{c|}{161}      & 1,294   & \multicolumn{1}{c|}{1.6}        & 8,839   \\ \hline
FLD        & \multicolumn{1}{c|}{210}      & 1,883   & \multicolumn{1}{c|}{0.82}       & 11,981  \\ \hline
OD         & \multicolumn{1}{c|}{149}      & 1,059   & \multicolumn{1}{c|}{13.2}       & 5,989    \\ \hline
TS         & \multicolumn{1}{c|}{152}      & 2,335   & \multicolumn{1}{c|}{1.6}        & 16,744     \\ \hline
\end{tabular}}
\end{table}
